Simulations of the formation and evolution of isolated dwarf galaxies - II. Angular momentum as a second parameter

We show results based on a large suite of N-Body/SPH simulations of isolated, flat dwarf galaxies, both rotating and non-rotating. The main goal is to investigate possible mechanisms to explain the observed dichotomy in radial stellar metallicity profiles of dwarf galaxies: dwarf irregulars (dIrr) and flat, rotating dwarf ellipticals (dE) generally possess flat metallicity profiles, while rounder and non-rotating dEs show strong negative metallicity gradients. These simulations show that flattening by rotation is key to reproducing the observed characteristics of flat dwarf galaxies, proving particularly efficient in erasing metallicity gradients. We propose a "centrifugal barrier mechanism" as an alternative to the previously suggested "fountain mechanism" for explaining the flat metallicity profiles of dIrrs and flat, rotating dEs. While only flattening the dark-matter halo has little influence, the addition of angular momentum slows down the infall of gas, so that star formation (SF) and the ensuing feedback are less centrally concentrated, occurring galaxy-wide. Additionally, this leads to more continuous SFHs by preventing large-scale oscillations in the SFR ("breathing"), and creates low density holes in the ISM, in agreement with observations of dIrrs. Our general conclusion is that rotation has a significant influence on the evolution and appearance of dwarf galaxies, and we suggest angular momentum as a second parameter (after galaxy mass as the dominant parameter) in dwarf galaxy evolution. Angular momentum differentiates between SF modes, making our fast rotating models qualitatively resemble dIrrs, which does not seem possible without rotation.

==> article_summary.tex <==
\section{summary}
\label{section:summary}

summary of all that has been written

